Sparse and weak-measurement certification of graph-edge entanglement in PXP scar wavepackets

An imperfect many-body revival does not by itself certify the entanglement of the returning state. We give a finite-record protocol for graph-edge localizable entanglement along scar wavepackets of a graph-dressed PXP chain. The target cluster state has nonzero energy variance, so neither an exact target eigenstate nor a dark-state embedding is assumed. Fresh binary probes of the undeformed Hamiltonians Pauli terms have a fully separable explanation, even within the dressed blockade sector. Adding local graph-stabilizer probes makes established entanglement witnesses accessible with simultaneous confidence bounds. For a specified square-root instrument, an imposed worst-case disturbance budget fixes the strength that minimizes the equal-allocation Hoeffding sufficient sampling cost. A local commutator bound accounts for finite-duration ancilla pulses while the Hamiltonian remains active. We test the protocol on chains through twenty spins, under perturbed dynamics, and with independent implementations. At the first twenty-spin return, synthetic weak records certify all nineteen graph edges. Generator, two-color, bounded-weight, and full-group benchmarks separate this localizable resource from genuine multipartite certification. The protocol measures recoverable entanglement in a known scar wavepacket, with explicit calibration and limits on its physical and statistical interpretation.

==> main_figure_numbers.tex <==
% Generated by code/sync_layout_refs.py from the compiled main.aux.
\newcommand{\MainProtocolFigure}{1}
\newcommand{\MainScarFigure}{2}
\newcommand{\MainExtendedFigure}{3}
\newcommand{\MainCertificationFigure}{4}
\newcommand{\MainGlobalFigure}{5}
\newcommand{\MainRobustnessFigure}{6}
\newcommand{\MainBudgetFigure}{7}
\newcommand{\MainInstrumentFigure}{8}

